GarmentCodeData: A Dataset of 3D Made-to-Measure Garments With Sewing Patterns

Recent research interest in the learning-based processing of garments, from virtual fitting to generation and reconstruction, stumbles on a scarcity of high-quality public data in the domain. We contribute to resolving this need by presenting the first large-scale synthetic dataset of 3D made-to-measure garments with sewing patterns, as well as its generation pipeline. GarmentCodeData contains 115,000 data points that cover a variety of designs in many common garment categories: tops, shirts, dresses, jumpsuits, skirts, pants, etc., fitted to a variety of body shapes sampled from a custom statistical body model based on CAESAR, as well as a standard reference body shape, applying three different textile materials. To enable the creation of datasets of such complexity, we introduce a set of algorithms for automatically taking tailor's measures on sampled body shapes, sampling strategies for sewing pattern design, and propose an automatic, open-source 3D garment draping pipeline based on a fast XPBD simulator, while contributing several solutions for collision resolution and drape correctness to enable scalability. Project Page: https://igl.ethz.ch/projects/GarmentCodeData/

==> fig_tex/body_segmentation.tex <==
\setlength{\columnsep}{10pt}%
\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{R}{0.2\linewidth}%
  \includegraphics[width=\linewidth]{fig/draping/segmentation.pdf}%
  \caption{Body model segmentation}
  \label{fig:body_seg}%
\end{wrapfigure}%

==> fig_tex/evaluation_measurements.tex <==
\begin{figure*}
  \centering
  % L, B, R, Top
  \includegraphics[trim=0cm 0cm 0cm -0.6cm,clip,width=0.98\linewidth,grid=false]{fig/evaluation/measurements/error_boxplot.png}
  \caption{Differences with the annotated measurements of the CAESAR data set. A positive error corresponds to an overestimation of our method; a negative one to an underestimation.} 
  \label{fig:eva_measurements_error_box}
\end{figure*}

==> fig_tex/measurement_lines.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\linewidth,height=14em,keepaspectratio]{fig/measurements/lines/circumferences.png}
    \includegraphics[width=0.56\linewidth,height=14em,keepaspectratio]{fig/measurements/lines/part_of_lines.png}
    \caption{\mk{Main body measurements.}}
    \label{fig:measurement_lines}
\end{figure}

==> fig_tex/stitching.tex <==
\setlength{\columnsep}{10pt}%
\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{r}{0.25\linewidth}%
  \includegraphics[width=\linewidth]{fig/draping/stitching_illustration.pdf}%
  \vspace{-0.2cm}
  \caption{Stitch matching directions. The correct match is shown in dark blue.}
  \label{fig:stitching}%
\end{wrapfigure}%
